Conditional Recurrent Flow: Conditional Generation of Longitudinal Samples with Applications to Neuroimaging

Generative models using neural network have opened a door to large-scale studies for various application domains, especially for studies that suffer from lack of real samples to obtain statistically robust inference. Typically, these generative models would train on existing data to learn the underlying distribution of the measurements (e.g., images) in latent spaces conditioned on covariates (e.g., image labels), and generate independent samples that are identically distributed in the latent space. Such models may work for cross-sectional studies, however, they are not suitable to generate data for longitudinal studies that focus on "progressive" behavior in a sequence of data. In practice, this is a quite common case in various neuroimaging studies whose goal is to characterize a trajectory of pathologies of a specific disease even from early stages. This may be too ambitious especially when the sample size is small (e.g., up to a few hundreds). Motivated from the setup above, we seek to develop a conditional generative model for longitudinal data generation by designing an invertable neural network. Inspired by recurrent nature of longitudinal data, we propose a novel neural network that incorporates recurrent subnetwork and context gating to include smooth transition in a sequence of generated data. Our model is validated on a video sequence dataset and a longitudinal AD dataset with various experimental settings for qualitative and quantitative evaluations of the generated samples. The results with the AD dataset captures AD specific group differences with sufficiently generated longitudinal samples that are consistent with existing literature, which implies a great potential to be applicable to other disease studies.

==> test.tex <==
\section{Goal}
\begin{itemize}
	\item (1) Invertible (2) sequential (3) conditional model
	\item Given: 
\begin{enumerate}
	\item Input sequence $X = x^{(1)},\dots,x^{(T)}$ (e.g., connectivity sequence, video, etc.)
	\item Corresponding covariates $Y = y^{(1)},\dots,y^{(T)}$ (e.g., age, gender, cognition, action label, class label, etc.)
\end{enumerate}
	\item Do:
	\begin{enumerate}
		\item Derive its sequential latent variables $Z = z^{(1)},\dots,z^{(T)}$
		\item With a $Z$ derived from $X$, change the covariates (at each $t$ or for all $t$) then generate a new sequence $X'$ (e.g., same subject, new trajectory conditioned on arbitrary cognition scores)
		\item If $Z$ is sampled such that $z^{(t)} \sim N(0,1)$ (while keeping $Y$), generate similar sequences $X'$.
		\item \textit{Exact invertible} process with scale/location operations.
		\item Then, for whatever generated $X'$, estimate the sequential densities $P_\mathcal{X}(X') = P_\mathcal{X}(x'^{(1)}), \dots, P_\mathcal{X}(x'^{(T)})$.
		\item Easy computation of Jacobian determinant for fast density estimation.
	\end{enumerate}
\end{itemize}

\section{Normal (Conditional) Inversion (Dinh et al., Ardizzone et al.)}
The goal is to approximate $p(x|y,z)$ where $y$ is an observable measurement (e.g., covariates, classes, etc.) and $z$ is a latent variable. Regardless of how $x$ is sampled, if we have an invertible function $f_\theta(x) = [y,z]$ such that $x = f_\theta^{-1}(y, z)$, we can sample $z \sim P_\mathcal{Z}(z)$ and exactly derive $x$:
\begin{equation}
x = g_\theta(y,z).
\end{equation}

An invertible architecture acts as an invertible function $f_\theta=g_\theta^{-1}$. Notice the network parameters $\theta$ is the same for both $f$ and $g$ implying that this is a single network trained in a bi-directional manner. Both $y$ and $z$ are computed with this network without two separate networks:
\begin{equation}
[y,z] = f_\theta(x) = [f_\theta^y(x), f_\theta^z(x)] = g_\theta^{-1}(x).
\end{equation}
For dimensionality differences, padding seems to be useful.

Then, there are mainly two cases to consider: (1) given $x$ and $y$, compute $z=f_\theta^z(x)$ and estimate $P_\mathcal{X}(x)$ and (2) sample $z$ and estimate $P_\mathcal{X}(x)$ with the $y$ of interest:
\begin{align}
P_\mathcal{X}(x) &= P_\mathcal{Z}(z)|\det(J^{-1})| \\
&=  P_\mathcal{Z}(f_\theta^z(x))\left|\det \left( \frac{\partial z}{\partial x} \right) \right| =  P_\mathcal{Z}(f_\theta^z(x))\left|\det \left( \frac{\partial f_\theta^z(x)}{\partial x} \right) \right| \quad \textrm{(given $x$)}\\
&= P_\mathcal{Z}(z)\left|\det \left( \frac{\partial x}{\partial [y,z]} \right)^{-1} \right| = P_\mathcal{Z}(z)\left|\det \left( \frac{\partial g_\theta(y,z)}{\partial [y,z]} \right)^{-1} \right| \quad \textrm{(sample $z$)}
\end{align}
Regardless of the case, $|J|$ can be computed solely based on the scale function $s$. The following is when there is only one block (no alternation):
\begin{equation}
\det \left( \frac{\partial f_\theta(x)}{\partial x} \right)= \exp \left[ \sum_k s_k(u_1) \right]
\end{equation}
for all $k$ entries of the first partition $u_1$ of $x$. With the alternation (coupling), use the fact that
\begin{equation}
\det(AB) = \det(A) \det(B).
\end{equation}
The inversion also works
\begin{equation}
(f_1 \circ f_2)^{-1} = f_1^{-1} \circ f_2^{-1}
\end{equation}

\section{Conditional Sequential Inversion?}
Extend the above formulations to sequential setting. We want to approximate $p(x^{(j)} | y^{(j)}, z^{(j)})$ for each time point $j = 1, \dots, J$. In other words, we need an invertible function $f_\theta(x^{(j)}) = [ y^{(j)}, z^{(j)}]$ such that
\begin{equation}
x^{(j)} = g_\theta(y^{(j)}, z^{(j)})
\end{equation}
is possible. But this does not utilize any sequential aspect of the data so all the time points are independent from each other except for the fact that the same model parameters $\theta$ are used. A more ideal setting would be to somehow use the previous sequence information $z^{(j-1)}$:
\begin{equation}
x^{(j)} = g_\theta(y^{(j)}, z^{(j)}, z^{(j-1)})
\end{equation}
where $z^{(j-1)}$ is the latent variable for the previous time point. Note that depending on how this is derived, it may contain knowledge about just the previous $j-1$ (i.e., each $z^{(j)}$ is derived independently), or it may be contain all the previous sequence information (i.e., each $z^{(j)}$ is sequentially derived).

How should we incorporate the latent information from other time points? We let the intermediate neural network components to incorporate this latent information. In other words, the scaling and translation functions can be neural networks that can \textit{explicitly} incorporate latent representations
\begin{equation}
v_1^{(j)} = u_1^{(j)} \otimes \exp(s_2(u_2^{(j)}, z^{(j-1)}) + t_2(u_2^{(j)}, z^{(j-1)})
\end{equation}
which is for the first block $u_1$. For the first time point $j=1$, $z^{(0)}$ can be some random/fixed initial latent variable which is commonly used in other sequential models.

Now, the new function $f_\theta(x^{(j)})$ can be represented similarly with the inclusion of a latent variable as a new argument:
\begin{equation}
[y^{(j)},z^{(j)}] = f_\theta(x^{(j)},z^{(j-1)}) = [f_\theta^y(x^{(j)},z^{(j-1)}), f_\theta^z(x^{(j)},z^{(j-1)})] = g_\theta^{-1}(x^{(j)},z^{(j-1)}).
\end{equation}
The inversion is trivial since even with the new networks with $z^{(j-1)}$, we consistently use the network to perform the same forward process. For instance, suppose we are given $X$ (and some $Y$). Once we sequentially generate $[y^{(j)},z^{(j)}]$ to construct $Z$, we can still perfectly reconstruct $X$ by generating $x^{(j)}$ sequentially with the same $Z$. This process is still guaranteed as long as the networks are used in the same order.

How about the Jacobian? Now it also depends on $z^{(j-1)}$ which makes it ``conditional'' on the previous sequences. Since the Jacobian determinant is merely a volume ``ratio'' between two distributions transformed by a function of interest, this function need not be static. The previous latent information is used as a ``function parameter'', no different from $\theta$. In that sense, it may be more appropriate to express $f_\theta^z(x^{(j)},z^{(j-1)})$ as $f_{\theta,z^{(j-1)}}^z(x^{(j)})$ to be explicit about how the function only maps $x^{(j)}$ to $z^{(j)}$.
\begin{align}
P_\mathcal{X}(x^{(j)}) &= P_\mathcal{Z}(z^{(j)})|\det(J^{-1})| \\
&=  P_\mathcal{Z}(f_{\theta,z^{(j-1)}}^z(x^{(j)}))\left|\det \left( \frac{\partial z^{(j)}}{\partial x^{(j)}} \right) \right| \\
&=  P_\mathcal{Z}(f_{\theta,z^{(j-1)}}^z(x^{(j)}))\left|\det \left( \frac{\partial f_{\theta,z^{(j-1)}}^z(x^{(j)})}{\partial x^{(j)}} \right) \right| \quad \textrm{(given $x^{(j)}$)}\\
&= P_\mathcal{Z}(z^{(j)})\left|\det \left( \frac{\partial x^{(j)}}{\partial [y^{(j)},z^{(j)}]} \right)^{-1} \right| \\
&= P_\mathcal{Z}(z^{(j)})\left|\det \left( \frac{\partial g_{\theta,z^{(j-1)}}(y^{(j)},z^{(j)})}{\partial [y^{(j)},z^{(j)}]} \right)^{-1} \right| \quad \textrm{(sample $z^{(j)}$)}
\end{align}

\subsection{Possible Networks}
Any network model that naturally make use of latent variables should work. Although the full model resembles a recurrent-type model, depending on how much we want the previous latent variables to be informative of the past, it may not even need to be RNN models. If we were to use a RNN model for $s$ and $t$, GRU seems reasonable since the cell actually only outputs the latent representations ($h$ which is like $z$ we want), which is exactly what we want. At least on Moving MNIST, GRU gets the job done. This is one place where we can be creative.



\section{Architecture}
Variables at time $j$ and partitions $k=1,2$:
\begin{enumerate}
	\item \textbf{Input}: $x^{(j)} \in \R^d$
	\item \textbf{Latent variable}: $z^{(j)} \in \R^{d_z}$
	\item \textbf{Conditional variable}: $y^{(j)} \in \R^{d_y}$ where $d_x = d_y + d_z$
	\item \textbf{Partitioned inputs}: $u_k^{(j)}\in \R^{d_{u_k}}$ where $d_x = d_{u_1} + d_{u_2}$
	\item \textbf{Partitioned outputs}: $v_k^{(j)}\in \R^{d_{u_k}}$
	\item \textbf{Scale functions}: $s_1(u_1^{(j)}, z^{(j-1)}): d_{u_1} \times d_z \rightarrow d_{u_2}$ and $s_2(u_2^{(j)}, z^{(j-1)}): d_{u_2} \times d_z \rightarrow d_{u_1}$ (notice the cross-mapping from $u_1$ to $u_2$, vice versa)
	\item \textbf{Translation functions}: $t_1(u_1^{(j)}, z^{(j-1)}): d_{u_1} \times d_z \rightarrow d_{u_2}$ and $t_2(u_2^{(j)}, z^{(j-1)}): d_{u_2} \times d_z \rightarrow d_{u_1}$ (notice the cross-mapping from $u_1$ to $u_2$, vice versa)
\end{enumerate}

\subsection{Forward Mapping}
\begin{equation}
v_1^{(j)} = u_1^{(j)} \otimes \exp(s_2(u_2^{(j)}, z^{(j-1)}) + t_2(u_2^{(j)}, z^{(j-1)})
\end{equation}
\begin{equation}
v_2^{(j)} = u_2^{(j)} \otimes \exp(s_1(v_1^{(j)}, z^{(j-1)}) + t_1(v_1^{(j)}, z^{(j-1)})
\end{equation}


\subsection{Inverse Mapping}
Note the covariates $y^{(j)}$ are part of $v^{(j)} = [v_1^{(j)}, v_2^{(j)}]$.
\begin{equation}
u_2^{(j)} = (v_2^{(j)} - t_1(v_1^{(j)}, z^{(j-1)})) \otimes \exp(-s_1(v_1^{(j)}, z^{(j-1)})
\end{equation}
\begin{equation}
u_1^{(j)} = (v_1^{(j)} - t_2(u_2^{(j)}, z^{(j-1)})) \otimes \exp(-s_2(u_2^{(j)}, z^{(j-1)})
\end{equation}

\setlength{\textfloatsep}{5pt}% Remove \textfloatsep
\begin{algorithm}[!t]
\caption{\label{alg:rprop} Conditional Invertible RNN (Post-Training)}
\begin{algorithmic}
\STATE \textbf{Given:}
\STATE 1) Sequence $X$
\STATE 2) Observed variables $Y$ (Optional)
\STATE 3) Sampled $Z$ (Optional)
\FOR{$j=1,2,\dots T$}
    \STATE $[y^{(j)},z^{(j)}] = f_\theta(x^{(j)},z^{(j-1)})$
    \STATE ehh....
\ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{figs/fig1.png}
\caption{An example for $j=1$ to $j=2$ with one coupling.}
\end{figure}
